STDepthFormer: Predicting Spatio-temporal Depth from Video with a Self-supervised Transformer Model

In this paper, a self-supervised model that simultaneously predicts a sequence of future frames from video-input with a novel spatial-temporal attention (ST) network is proposed. The ST transformer network allows constraining both temporal consistency across future frames whilst constraining consistency across spatial objects in the image at different scales. This was not the case in prior works for depth prediction, which focused on predicting a single frame as output. The proposed model leverages prior scene knowledge such as object shape and texture similar to single-image depth inference methods, whilst also constraining the motion and geometry from a sequence of input images. Apart from the transformer architecture, one of the main contributions with respect to prior works lies in the objective function that enforces spatio-temporal consistency across a sequence of output frames rather than a single output frame. As will be shown, this results in more accurate and robust depth sequence forecasting. The model achieves highly accurate depth forecasting results that outperform existing baselines on the KITTI benchmark. Extensive ablation studies were performed to assess the effectiveness of the proposed techniques. One remarkable result of the proposed model is that it is implicitly capable of forecasting the motion of objects in the scene, rather than requiring complex models involving multi-object detection, segmentation and tracking.

==> backup.tex <==

@inproceedings{safadoust2021self,
  title={Self-Supervised Monocular Scene Decomposition and Depth Estimation},
  author={Safadoust, Sadra and G{\"u}ney, Fatma},
  booktitle={2021 International Conference on 3D Vision (3DV)},
  pages={627--636},
  year={2021},
  organization={IEEE}
}

@inproceedings{lee2021attentive,
  title={Attentive and contrastive learning for joint depth and motion field estimation},
  author={Lee, Seokju and Rameau, Francois and Pan, Fei and Kweon, In So},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4862--4871},
  year={2021}
}

@inproceedings{hur2020self,
  title={Self-supervised monocular scene flow estimation},
  author={Hur, Junhwa and Roth, Stefan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7396--7405},
  year={2020}
}

%%%%%%%%% Transfomers %%%%%%%%%%
@article{cheng2021masked,
  title={Masked-attention mask transformer for universal image segmentation},
  author={Cheng, Bowen and Misra, Ishan and Schwing, Alexander G and Kirillov, Alexander and Girdhar, Rohit},
  journal={arXiv preprint arXiv:2112.01527},
  year={2021}
}
@article{li2021grounded,
  title={Grounded Language-Image Pre-training},
  author={Li, Liunian Harold and Zhang, Pengchuan and Zhang, Haotian and Yang, Jianwei and Li, Chunyuan and Zhong, Yiwu and Wang, Lijuan and Yuan, Lu and Zhang, Lei and Hwang, Jenq-Neng and others},
  journal={arXiv preprint arXiv:2112.03857},
  year={2021}
}

@article{li2021improved,
  title={Improved multiscale vision transformers for classification and detection},
  author={Li, Yanghao and Wu, Chao-Yuan and Fan, Haoqi and Mangalam, Karttikeya and Xiong, Bo and Malik, Jitendra and Feichtenhofer, Christoph},
  journal={arXiv preprint arXiv:2112.01526},
  year={2021}
}

@article{zhai2021scaling,
  title={Scaling vision transformers},
  author={Zhai, Xiaohua and Kolesnikov, Alexander and Houlsby, Neil and Beyer, Lucas},
  journal={arXiv preprint arXiv:2106.04560},
  year={2021}
}

@article{raffel2019exploring,
  title={Exploring the limits of transfer learning with a unified text-to-text transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={arXiv preprint arXiv:1910.10683},
  year={2019}
}
@inproceedings{Vaswani,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 publisher = {Curran Associates, Inc.},
 title = {Attention is All you Need},
 volume = {30},
 year = {2017}
}

@article{Devlin2019,
archivePrefix = {arXiv},
arxivId = {1810.04805},
author = {Devlin, Jacob and Chang, Ming Wei and Lee, Kenton and Toutanova, Kristina},
eprint = {1810.04805},
isbn = {9781950737130},
journal = {NAACL HLT 2019 - 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies - Proceedings of the Conference},
number = {Mlm},
pages = {4171--4186},
title = {{BERT: Pre-training of deep bidirectional transformers for language understanding}},
volume = {1},
year = {2019}
}
@article{Brown2020,
archivePrefix = {arXiv},
arxivId = {2005.14165},
author = {Brown, Tom B. and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel M. and Wu, Jeffrey and Winter, Clemens and Hesse, Christopher and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
eprint = {2005.14165},
issn = {10495258},
journal = {Advances in Neural Information Processing Systems},
title = {{Language models are few-shot learners}},
volume = {2020-December},
year = {2020}
}

@article{dosovitskiy2020,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}
@article{Liu2021,
  title={Swin transformer: Hierarchical vision transformer using shifted windows},
  author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  journal={arXiv preprint arXiv:2103.14030},
  year={2021}
}



%%%% VIDEO FORECASTING %%%%%%%%%%%%%%%%%%%µ

@inproceedings{Eigena,
archivePrefix = {arXiv},
arxivId = {1411.4734},
author = {Eigen, David and Fergus, Rob},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2015.304},
eprint = {1411.4734},
isbn = {9781467383912},
issn = {15505499},
pages = {2650--2658},
title = {{Predicting depth, surface normals and semantic labels with a common multi-scale convolutional architecture}},
volume = {2015 Inter},
year = {2015}
}
@inproceedings{Eigen,
archivePrefix = {arXiv},
arxivId = {1406.2283},
author = {Eigen, David and Puhrsch, Christian and Fergus, Rob},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1406.2283},
issn = {10495258},
pages = {2366--2374},
title = {{Depth map prediction from a single image using a multi-scale deep network}},
volume = {3},
year = {2014}
}


@inproceedings{WilliamLotter2016,
archivePrefix = {arXiv},
arxivId = {1605.07157},
author = {{William Lotter}, Gabriel Kreiman and David Cox},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1605.07157},
issn = {10495258},
pages = {64--72},
title = {{Deep Predictive Coding Networks for Video Prediction and Unsupervised Learning}},
year = {2016}
}
@inproceedings{Wang2020a,
archivePrefix = {arXiv},
arxivId = {2008.05861},
author = {Wang, Jiangliu and Jiao, Jianbo and Liu, Yun Hui},
booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
doi = {10.1007/978-3-030-58520-4_30},
eprint = {2008.05861},
isbn = {9783030585198},
issn = {16113349},
keywords = {Pace,Self-supervised learning,Unsupervised,Video representation},
pages = {504--521},
title = {{ContextVP: Fully Context-Aware Video Prediction}},
volume = {12362 LNCS},
year = {2020}
}
@inproceedings{Finn,
archivePrefix = {arXiv},
arxivId = {1605.07157},
author = {Finn, Chelsea and Goodfellow, Ian and Levine, Sergey},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1605.07157},
issn = {10495258},
pages = {64--72},
title = {{Unsupervised learning for physical interaction through video prediction}},
year = {2016}
}

@article{Kumar2019,
  title={Videoflow: A conditional flow-based model for stochastic video generation},
  author={Kumar, Manoj and Babaeizadeh, Mohammad and Erhan, Dumitru and Finn, Chelsea and Levine, Sergey and Dinh, Laurent and Kingma, Durk},
  journal={arXiv preprint arXiv:1903.01434},
  year={2019}
}

@article{Wu2021a,
archivePrefix = {arXiv},
arxivId = {2103.04174},
author = {Wu, Bohan and Nair, Suraj and Martin-Martin, Roberto and Fei-Fei, Li and Finn, Chelsea},
eprint = {2103.04174},
title = {{Greedy Hierarchical Variational Autoencoders for Large-Scale Video Prediction}},
year = {2021}
}
@inproceedings{Ye2019,
archivePrefix = {arXiv},
arxivId = {1908.08522},
author = {Ye, Yufei and Singh, Maneesh and Gupta, Abhinav and Tulsiani, Shubham},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2019.01045},
eprint = {1908.08522},
isbn = {9781728148038},
issn = {15505499},
pages = {10352--10361},
title = {{Compositional video prediction}},
volume = {2019-Octob},
year = {2019}
}
@inproceedings{Reda2021,
archivePrefix = {arXiv},
arxivId = {1811.00684},
author = {Reda, Fitsum A and Liu, Guilin and Shih, Kevin J and Kirby, Robert and Barker, Jon and Tarjan, David and Tao, Andrew and Catanzaro, Bryan},
booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
doi = {10.1007/978-3-030-01234-2_44},
eprint = {1811.00684},
isbn = {9783030012335},
issn = {16113349},
keywords = {3D CNN,Frame prediction,Optical flow,Sampling kernel},
pages = {747--763},
title = {{SDC-Net: Video prediction using spatially-displaced convolution}},
volume = {11211 LNCS},
year = {2018}
}
@inproceedings{Kalchbrenner2017,
archivePrefix = {arXiv},
arxivId = {1610.00527},
author = {Kalchbrenner, Nal and {Van Den Oord}, A{\"{a}}ron and Simonyan, Karen and Danihelka, Ivo and Vinyals, Oriol and Graves, Alex and Kavukcuoglu, Koray},
booktitle = {34th International Conference on Machine Learning, ICML 2017},
eprint = {1610.00527},
isbn = {9781510855144},
pages = {2821--2829},
title = {{Video pixel networks}},
volume = {4},
year = {2017}
}
@inproceedings{Gao2019,
archivePrefix = {arXiv},
arxivId = {1812.00452},
author = {Gao, Hang and Xu, Huazhe and Cai, Qi Zhi and Wang, Ruth and Yu, Fisher and Darrell, Trevor},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2019.00910},
eprint = {1812.00452},
isbn = {9781728148038},
issn = {15505499},
pages = {9005--9014},
title = {{Disentangling propagation and generation for video prediction}},
volume = {2019-Octob},
year = {2019}
}
@inproceedings{Babaeizadeh2018,
archivePrefix = {arXiv},
arxivId = {1710.11252},
author = {Babaeizadeh, Mohammad and Finn, Chelsea and Erhan, Dumitru and Campbell, Roy and Levine, Sergey},
booktitle = {6th International Conference on Learning Representations, ICLR 2018 - Conference Track Proceedings},
eprint = {1710.11252},
isbn = {1710.11252v2},
title = {{Stochastic variational video prediction}},
year = {2018}
}
@inproceedings{Denton2018,
archivePrefix = {arXiv},
arxivId = {1802.07687},
author = {Denton, Emily and Fergus, Rob},
booktitle = {35th International Conference on Machine Learning, ICML 2018},
eprint = {1802.07687},
isbn = {9781510867963},
pages = {1906--1919},
title = {{Stochastic Video Generation with a Learned Prior}},
volume = {3},
year = {2018}
}
@article{Yan2021,
archivePrefix = {arXiv},
arxivId = {2104.10157},
author = {Yan, Wilson and Zhang, Yunzhi and Abbeel, Pieter and Srinivas, Aravind},
eprint = {2104.10157},
title = {{VideoGPT: Video Generation using VQ-VAE and Transformers}},
year = {2021}
}


@article{Walker2021,
  title={Predicting Video with VQVAE},
  author={Walker, Jacob and Razavi, Ali and Oord, A{\"a}ron van den},
  journal={arXiv preprint arXiv:2103.01950},
  year={2021}
}


@inproceedings{Wu2021,
  title={MotionRNN: A flexible model for video prediction with spacetime-varying motions},
  author={Wu, Haixu and Yao, Zhiyu and Wang, Jianmin and Long, Mingsheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15435--15444},
  year={2021}
}






%%%% SEMANTIC FORECASTING %%%%%%%%%%%%%%%%%%%µ


@inproceedings{Terwilliger2019,
archivePrefix = {arXiv},
arxivId = {1809.08318},
author = {Terwilliger, Adam M and Brazil, Garrick and Liu, Xiaoming},
booktitle = {Proceedings - 2019 IEEE Winter Conference on Applications of Computer Vision, WACV 2019},
doi = {10.1109/WACV.2019.00186},
eprint = {1809.08318},
isbn = {9781728119755},
pages = {1703--1712},
title = {{Recurrent flow-guided semantic forecasting}},
year = {2019}
}


@inproceedings{Bhattacharyya2019,
archivePrefix = {arXiv},
arxivId = {1810.00746},
author = {Bhattacharyya, Apratim and Fritz, Mario and Schiele, Bernt},
booktitle = {7th International Conference on Learning Representations, ICLR 2019},
eprint = {1810.00746},
title = {{Bayesian prediction of future street scenes using synthetic likelihoods}},
year = {2019}
}


@inproceedings{Luc2017,
archivePrefix = {arXiv},
arxivId = {1703.07684},
author = {Luc, Pauline and Neverova, Natalia and Couprie, Camille and Verbeek, Jakob and Lecun, Yann},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2017.77},
eprint = {1703.07684},
isbn = {9781538610329},
issn = {15505499},
pages = {648--657},
title = {{Predicting Deeper into the Future of Semantic Segmentation}},
volume = {2017-Octob},
year = {2017}
}


@inproceedings{Graber2021,
archivePrefix = {arXiv},
arxivId = {2104.03962},
author = {Graber, Colin and Tsai, Grace and Firman, Michael and Brostow, Gabriel and Schwing, Alexander},
booktitle = {IEEE Computer Society Conference on Computer Vision and Pattern Recognition Workshops},
doi = {10.1109/CVPRW53098.2021.00257},
eprint = {2104.03962},
isbn = {9781665448994},
issn = {21607516},
pages = {2279--2288},
title = {{Panoptic segmentation forecasting}},
year = {2021}
}


@article{Chiu2020,
archivePrefix = {arXiv},
arxivId = {1904.10666},
author = {Chiu, Hsu Kuang and Adeli, Ehsan and Niebles, Juan Carlos},
doi = {10.1109/LRA.2020.2992184},
eprint = {1904.10666},
issn = {23773766},
journal = {IEEE Robotics and Automation Letters},
keywords = {Computer vision for transportation,deep learning for visual perception,semantic scene understanding,visual learning},
number = {3},
pages = {4202--4209},
title = {{Segmenting the Future}},
volume = {5},
year = {2020}
}



@inproceedings{Saric2020,
author = {Saric, Josip and Orsic, Marin and Antunovic, Tonci and Vrazic, Sacha and Segvic, Sinisa},
booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
doi = {10.1109/CVPR42600.2020.01066},
issn = {10636919},
pages = {10645--10654},
title = {{Warp to the Future: Joint Forecasting of Features and Feature Motion}},
year = {2020}
}
@article{Mathieu2016,
  title={Deep multi-scale video prediction beyond mean square error},
  author={Mathieu, Michael and Couprie, Camille and LeCun, Yann},
  journal={arXiv preprint arXiv:1511.05440},
  year={2015}
}

@inproceedings{Rakhimov,
archivePrefix = {arXiv},
arxivId = {2006.10704},
author = {Rakhimov, Ruslan and Volkhonskiy, Denis and Artemov, Alexey and Zorin, Denis and Burnaev, Evgeny},
booktitle = {VISIGRAPP 2021 - Proceedings of the 16th International Joint Conference on Computer Vision, Imaging and Computer Graphics Theory and Applications},
doi = {10.5220/0010241801010112},
eprint = {2006.10704},
isbn = {9789897584886},
keywords = {Deep learning,Generative adversarial networks,Video generation},
pages = {101--112},
title = {{Latent video transformer}},
volume = {5},
year = {2021}
}


%%%% DEPTH FORECASTING %%%%%%%%%%%%%%%%%%%µ



@article{weng2020inverting,
  title={Inverting the Pose Forecasting Pipeline with SPF2: Sequential Pointcloud Forecasting for Sequential Pose Forecasting},
  author={Weng, Xinshuo and Wang, Jianren and Levine, Sergey and Kitani, Kris and Rhinehart, Nicholas},
  journal={arXiv preprint arXiv:2003.08376},
  year={2020}
}

@inproceedings{Mahjourian2017,
archivePrefix = {arXiv},
arxivId = {1609.06377},
author = {Mahjourian, Reza and Wicke, Martin and Angelova, Anelia},
booktitle = {IEEE Intelligent Vehicles Symposium, Proceedings},
doi = {10.1109/IVS.2017.7995953},
eprint = {1609.06377},
isbn = {9781509048045},
pages = {1700--1707},
title = {{Geometry-based next frame prediction from monocular video}},
year = {2017}
}

@inproceedings{Qi2019,
author = {Qi, Xiaojuan and Liu, Zhengzhe and Chen, Qifeng and Jia, Jiaya},
booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
doi = {10.1109/CVPR.2019.00786},
isbn = {9781728132938},
issn = {10636919},
keywords = {Image and Video Synthesis,RGBD sensors and analytics},
pages = {7665--7674},
title = {{3D motion decomposition for RGBD future dynamic scene synthesis}},
volume = {2019-June},
year = {2019}
}

@inproceedings{Hu2020,
archivePrefix = {arXiv},
arxivId = {2003.06409},
author = {Hu, Anthony and Cotter, Fergal and Mohan, Nikhil and Gurau, Corina and Kendall, Alex},
booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
doi = {10.1007/978-3-030-58517-4_45},
eprint = {2003.06409},
isbn = {9783030585167},
issn = {16113349},
pages = {767--785},
title = {{Probabilistic Future Prediction for Video Scene Understanding}},
volume = {12361 LNCS},
year = {2020}
}


%%%% DEPTH ESTIMATION %%%%%%%%%%%%%%%%%%%µ
@article{Yin2018,
archivePrefix = {arXiv},
arxivId = {1803.02276},
author = {Yin, Zhichao and Shi, Jianping},
doi = {10.1109/CVPR.2018.00212},
eprint = {1803.02276},
isbn = {9781538664209},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {1983--1992},
title = {{GeoNet: Unsupervised Learning of Dense Depth, Optical Flow and Camera Pose}},
year = {2018}
}
@article{Shu2020,
archivePrefix = {arXiv},
arxivId = {2007.10603},
author = {Shu, Chang and Yu, Kun and Duan, Zhixiang and Yang, Kuiyuan},
doi = {10.1007/978-3-030-58529-7_34},
eprint = {2007.10603},
isbn = {9783030585280},
issn = {16113349},
journal = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
pages = {572--588},
title = {{Feature-Metric Loss for Self-supervised Learning of Depth and Egomotion}},
volume = {12364 LNCS},
year = {2020}
}
@article{xu2021transcenter,
  title={Transcenter: Transformers with dense queries for multiple-object tracking},
  author={Xu, Yihong and Ban, Yutong and Delorme, Guillaume and Gan, Chuang and Rus, Daniela and Alameda-Pineda, Xavier},
  journal={arXiv preprint arXiv:2103.15145},
  year={2021}
}
@article{Wang2021,
author = {Wang, Lijun and Wang, Yifan and Wang, Linzhao and Zhan, Yunlong and Wang, Ying and Lu, Huchuan},
journal = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
pages = {12727--12736},
title = {{Can Scale-Consistent Monocular Depth Be Learned in a Self-Supervised Scale-Invariant Manner?}},
year = {2021}
}

@inproceedings{Ranjan2019,
arxivId = {1805.09806},
author = {Ranjan, Anurag and Jampani, Varun and Balles, Lukas and Kim, Kihwan and Sun, Deqing and Wulff, Jonas and Black, Michael J},
booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
doi = {10.1109/CVPR.2019.01252},
eprint = {1805.09806},
isbn = {9781728132938},
issn = {10636919},
keywords = {Deep Learning,Low-level Vision},
pages = {12232--12241},
title = {{Competitive collaboration: Joint unsupervised learning of depth, camera motion, optical flow and motion segmentation}},
volume = {2019-June},
year = {2019}
}
@misc{wu2019detectron2,
  author =       {Yuxin Wu and Alexander Kirillov and Francisco Massa and
                  Wan-Yen Lo and Ross Girshick},
  title =        {Detectron2},
  website = {\url{https://github.com/facebookresearch/detectron2}},
  year =         {2019}
}
@article{luo2019every,
  title={Every pixel counts++: Joint learning of geometry and motion with 3d holistic understanding},
  author={Luo, Chenxu and Yang, Zhenheng and Wang, Peng and Wang, Yang and Xu, Wei and Nevatia, Ram and Yuille, Alan},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={42},
  number={10},
  pages={2624--2641},
  year={2019},
  publisher={IEEE}
}


@inproceedings{xu2021moving,
  title={Moving slam: Fully unsupervised deep learning in non-rigid scenes},
  author={Xu, Dan and Vedaldi, Andrea and Henriques, Joao F},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4611--4617},
  year={2021},
  organization={IEEE}
}


@article{Yang2021,
archivePrefix = {arXiv},
arxivId = {2103.12091},
author = {Yang, Guanglei and Tang, Hao and Ding, Mingli and Sebe, Nicu and Ricci, Elisa},
eprint = {2103.12091},
pages = {16269--16279},
title = {{Transformer-Based Attention Networks for Continuous Pixel-Wise Prediction}},
year = {2021}
}
@article{Gordon2019,
archivePrefix = {arXiv},
arxivId = {1904.04998},
author = {Gordon, Ariel and Li, Hanhan and Jonschkowski, Rico and Angelova, Anelia},
doi = {10.1109/ICCV.2019.00907},
eprint = {1904.04998},
isbn = {9781728148038},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
pages = {8976--8985},
title = {{Depth from videos in the wild: Unsupervised monocular depth learning from unknown cameras}},
volume = {2019-Octob},
year = {2019}
}
@inproceedings{chen2019towards,
  title={Towards scene understanding: Unsupervised monocular depth estimation with semantic-aware representation},
  author={Chen, Po-Yi and Liu, Alexander H and Liu, Yen-Cheng and Wang, Yu-Chiang Frank},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2624--2632},
  year={2019}
}

@article{Kendall2015,
archivePrefix = {arXiv},
arxivId = {1505.07427},
author = {Kendall, Alex and Grimes, Matthew and Cipolla, Roberto},
doi = {10.1109/ICCV.2015.336},
eprint = {1505.07427},
isbn = {9781467383912},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
pages = {2938--2946},
title = {{PoseNet: A convolutional network for real-time 6-dof camera relocalization}},
volume = {2015 Inter},
year = {2015}
}
@inproceedings{chen2019self,
  title={Self-supervised learning with geometric constraints in monocular video: Connecting flow, depth, and camera},
  author={Chen, Yuhua and Schmid, Cordelia and Sminchisescu, Cristian},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={7063--7072},
  year={2019}
}
@article{mccraith2020monocular,
  title={Monocular depth estimation with self-supervised instance adaptation},
  author={McCraith, Robert and Neumann, Lukas and Zisserman, Andrew and Vedaldi, Andrea},
  journal={arXiv preprint arXiv:2004.05821},
  year={2020}
}
@article{Jaderberg2015,
archivePrefix = {arXiv},
arxivId = {1506.02025},
author = {Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and Kavukcuoglu, Koray},
eprint = {1506.02025},
issn = {10495258},
journal = {Advances in Neural Information Processing Systems},
pages = {2017--2025},
title = {{Spatial transformer networks}},
volume = {2015-Janua},
year = {2015}
}
@article{Mahjourian2018,
archivePrefix = {arXiv},
arxivId = {1802.05522},
author = {Mahjourian, Reza and Wicke, Martin and Angelova, Anelia},
doi = {10.1109/CVPR.2018.00594},
eprint = {1802.05522},
isbn = {9781538664209},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {5667--5675},
title = {{Unsupervised Learning of Depth and Ego-Motion from Monocular Video Using 3D Geometric Constraints}},
year = {2018}
}
@article{Liu2016,
archivePrefix = {arXiv},
arxivId = {1502.07411},
author = {Liu, Fayao and Shen, Chunhua and Lin, Guosheng and Reid, Ian},
doi = {10.1109/TPAMI.2015.2505283},
eprint = {1502.07411},
issn = {01628828},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
keywords = {Depth estimation,conditional random field (CRF),deep convolutional neural networks (CNN),fully convolutional networks,superpixel pooling},
number = {10},
pages = {2024--2039},
title = {{Learning Depth from Single Monocular Images Using Deep Convolutional Neural Fields}},
volume = {38},
year = {2016}
}


@article{Chen2016,
  title={Single-image depth perception in the wild},
  author={Chen, Weifeng and Fu, Zhao and Yang, Dawei and Deng, Jia},
  journal={Advances in neural information processing systems},
  volume={29},
  pages={730--738},
  year={2016}
}

@article{Godard2017,
archivePrefix = {arXiv},
arxivId = {1609.03677},
author = {Godard, Cl{\'{e}}ment and {Mac Aodha}, Oisin and Brostow, Gabriel J.},
doi = {10.1109/CVPR.2017.699},
eprint = {1609.03677},
isbn = {9781538604571},
issn = {1063-6919},
journal = {Proceedings - 30th IEEE Conference on Computer Vision and Pattern Recognition, CVPR 2017},
pages = {6602--6611},
title = {{Unsupervised monocular depth estimation with left-right consistency}},
volume = {2017-January},
year = {2017}
}
@article{Zhou2017,
archivePrefix = {arXiv},
arxivId = {1704.07813},
author = {Zhou, Tinghui and Brown, Matthew and Snavely, Noah and Lowe, David G.},
doi = {10.1109/CVPR.2017.700},
eprint = {1704.07813},
isbn = {9781538604571},
journal = {Proceedings - 30th IEEE Conference on Computer Vision and Pattern Recognition, CVPR 2017},
pages = {6612--6621},
title = {{Unsupervised learning of depth and ego-motion from video}},
volume = {2017-January},
year = {2017}
}
@inproceedings{garg2016unsupervised,
  title={Unsupervised cnn for single view depth estimation: Geometry to the rescue},
  author={Garg, Ravi and Bg, Vijay Kumar and Carneiro, Gustavo and Reid, Ian},
  booktitle={European conference on computer vision},
  pages={740--756},
  year={2016},
  organization={Springer}
}
@article{Zhan2018,
archivePrefix = {arXiv},
arxivId = {1803.03893},
author = {Zhan, Huangying and Garg, Ravi and Weerasekera, Chamara Saroj and Li, Kejie and Agarwal, Harsh and Reid, Ian M.},
doi = {10.1109/CVPR.2018.00043},
eprint = {1803.03893},
isbn = {9781538664209},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {340--349},
title = {{Unsupervised Learning of Monocular Depth Estimation and Visual Odometry with Deep Feature Reconstruction}},
year = {2018}
}
@article{Godard2019,
archivePrefix = {arXiv},
arxivId = {1806.01260},
author = {Godard, Clement and Aodha, Oisin Mac and Firman, Michael and Brostow, Gabriel},
doi = {10.1109/ICCV.2019.00393},
eprint = {1806.01260},
isbn = {9781728148038},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
number = {1},
pages = {3827--3837},
title = {{Digging into self-supervised monocular depth estimation}},
volume = {2019-October},
year = {2019}
}
@article{Chen2019,
archivePrefix = {arXiv},
arxivId = {1907.05820},
author = {Chen, Yuhua and Schmid, Cordelia and Sminchisescu, Cristian},
doi = {10.1109/ICCV.2019.00716},
eprint = {1907.05820},
isbn = {9781728148038},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
pages = {7062--7071},
title = {{Self-supervised learning with geometric constraints in monocular video: Connecting flow, depth, and camera}},
volume = {2019-October},
year = {2019}
}
@article{Lee2019,
archivePrefix = {arXiv},
arxivId = {1909.06999},
author = {Lee, Seokju and Im, Sunghoon and Lin, Stephen and Kweon, In So},
doi = {10.1109/IROS40897.2019.8967970},
eprint = {1909.06999},
isbn = {9781728140049},
issn = {21530866},
journal = {IEEE International Conference on Intelligent Robots and Systems},
pages = {1180--1186},
title = {{Learning Residual Flow as Dynamic Motion from Stereo Videos}},
year = {2019}
}
@article{Johnston2020,
archivePrefix = {arXiv},
arxivId = {2003.13951},
author = {Johnston, Adrian and Carneiro, Gustavo},
doi = {10.1109/CVPR42600.2020.00481},
eprint = {2003.13951},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {4755--4764},
title = {{Self-supervised monocular trained depth estimation using self-attention and discrete disparity volume}},
year = {2020}
}
@article{Klingner2020,
archivePrefix = {arXiv},
arxivId = {2007.06936},
author = {Klingner, Marvin and Term{\"{o}}hlen, Jan Aike and Mikolajczyk, Jonas and Fingscheidt, Tim},
doi = {10.1007/978-3-030-58565-5_35},
eprint = {2007.06936},
isbn = {9783030585648},
issn = {16113349},
journal = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
pages = {582--600},
title = {{Self-supervised Monocular Depth Estimation: Solving the Dynamic Object Problem by Semantic Guidance}},
volume = {12365 LNCS},
year = {2020}
}
@article{lou2020safenet,
  title={Safenet: Self-supervised monocular depth estimation with semantic-aware feature extraction},
  author={Choi, Jaehoon and Jung, Dongki and Lee, Donghwan and Kim, Changick},
  journal={arXiv preprint arXiv:2010.02893},
  year={2020}
}
@article{Bian2019,
  title={Unsupervised scale-consistent depth and ego-motion learning from monocular video},
  author={Bian, Jiawang and Li, Zhichao and Wang, Naiyan and Zhan, Huangying and Shen, Chunhua and Cheng, Ming-Ming and Reid, Ian},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={35--45},
  year={2019}
}
@inproceedings{johnston2020self,
  title={Self-supervised monocular trained depth estimation using self-attention and discrete disparity volume},
  author={Johnston, Adrian and Carneiro, Gustavo},
  booktitle={Proceedings of the ieee/cvf conference on computer vision and pattern recognition},
  pages={4756--4765},
  year={2020}
}
@inproceedings{Watson2021,
  title={The Temporal Opportunist: Self-Supervised Multi-Frame Monocular Depth},
  author={Watson, Jamie and Mac Aodha, Oisin and Prisacariu, Victor and Brostow, Gabriel and Firman, Michael},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1164--1174},
  year={2021}
}
@article{mohan2021efficientps,
  title={Efficientps: Efficient panoptic segmentation},
  author={Mohan, Rohit and Valada, Abhinav},
  journal={International Journal of Computer Vision},
  volume={129},
  number={5},
  pages={1551--1579},
  year={2021},
  publisher={Springer}
}
@article{meinhardt2021trackformer,
  title={Trackformer: Multi-object tracking with transformers},
  author={Meinhardt, Tim and Kirillov, Alexander and Leal-Taixe, Laura and Feichtenhofer, Christoph},
  journal={arXiv preprint arXiv:2101.02702},
  year={2021}
}
@inproceedings{tan2019efficientnet,
  title={Efficientnet: Rethinking model scaling for convolutional neural networks},
  author={Tan, Mingxing and Le, Quoc},
  booktitle={International conference on machine learning},
  pages={6105--6114},
  year={2019},
  organization={PMLR}
}
@article{chen2018searching,
  title={Searching for efficient multi-scale architectures for dense image prediction},
  author={Chen, Liang-Chieh and Collins, Maxwell and Zhu, Yukun and Papandreou, George and Zoph, Barret and Schroff, Florian and Adam, Hartwig and Shlens, Jon},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}
@inproceedings{he2017mask,
  title={Mask r-cnn},
  author={He, Kaiming and Gkioxari, Georgia and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2961--2969},
  year={2017}
}
@inproceedings{tan2020efficientdet,
  title={Efficientdet: Scalable and efficient object detection},
  author={Tan, Mingxing and Pang, Ruoming and Le, Quoc V},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={10781--10790},
  year={2020}
}
@article{Boulahbal2021,
  title={Are conditional GANs explicitly conditional?},
  author={Boulahbal, Houssem-eddine and Voicila, Adrian and Comport, Andrew},
  journal={arXiv preprint arXiv:2106.15011},
  year={2021}
}
@inproceedings{cordts2016cityscapes,
  title={The cityscapes dataset for semantic urban scene understanding},
  author={Cordts, Marius and Omran, Mohamed and Ramos, Sebastian and Rehfeld, Timo and Enzweiler, Markus and Benenson, Rodrigo and Franke, Uwe and Roth, Stefan and Schiele, Bernt},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3213--3223},
  year={2016}
}
@inproceedings{Almalioglu2019,
archivePrefix = {arXiv},
arxivId = {1809.05786},
author = {Almalioglu, Yasin and Saputra, Muhamad Risqi U. and {De Gusmao}, Pedro P.B. and Markham, Andrew and Trigoni, Niki},
booktitle = {Proceedings - IEEE International Conference on Robotics and Automation},
doi = {10.1109/ICRA.2019.8793512},
eprint = {1809.05786},
isbn = {9781538660263},
issn = {10504729},
pages = {5474--5480},
title = {{GANVO: Unsupervised deep monocular visual odometry and depth estimation with generative adversarial networks}},
volume = {2019-May},
year = {2019}
}
@article{vijayanarasimhan,
  title={Sfm-net: Learning of structure and motion from video},
  author={Vijayanarasimhan, Sudheendra and Ricco, Susanna and Schmid, Cordelia and Sukthankar, Rahul and Fragkiadaki, Katerina},
  journal={arXiv preprint arXiv:1704.07804},
  year={2017}
}

@article{lee2021learning,
  title={Learning monocular depth in dynamic scenes via instance-aware projection consistency},
  author={Lee, Seokju and Im, Sunghoon and Lin, Stephen and Kweon, In So},
  journal={arXiv preprint arXiv:2102.02629},
  year={2021}
}

@article{Lee2019a,
archivePrefix = {arXiv},
arxivId = {1907.10326},
author = {Lee, Jin Han and Han, Myung-kyu and Ko, Dong Wook and Suh, Il Hong},
eprint = {1907.10326},
issn = {2331-8422},
title = {{From Big to Small: Multi-Scale Local Planar Guidance for Monocular Depth Estimation}},
url = {http://arxiv.org/abs/1907.10326},
year = {2019}
}
@article{Rares2020,
archivePrefix = {arXiv},
arxivId = {1905.02693},
author = {Rares, Vitor Guizilini and Ambrus and Pillai, Sudeep and Raventos, Allan and Gaidon, Adrien},
doi = {10.1109/CVPR42600.2020.00256},
eprint = {1905.02693},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {2482--2491},
title = {{3D packing for self-supervised monocular depth estimation}},
year = {2020}
}
@article{Li2021,
archivePrefix = {arXiv},
arxivId = {2101.02143},
author = {Li, Xiangyu and Hou, Yonghong and Wang, Pichao and Gao, Zhimin and Xu, Mingliang and Li, Wanqing},
doi = {10.1007/s00521-020-05545-8},
eprint = {2101.02143},
issn = {14333058},
journal = {Neural Computing and Applications},
keywords = {Geometry constraint,Transformer,Unsupervised learning,Visual odometry},
number = {13},
pages = {8031--8042},
title = {{Transformer guided geometry model for flow-based unsupervised visual odometry}},
volume = {33},
year = {2021}
}
@inproceedings{yang2018unsupervised,
  title={Unsupervised learning of geometry from videos with edge-aware depth-normal consistency},
  author={Yang, Zhenheng and Wang, Peng and Xu, Wei and Zhao, Liang and Nevatia, Ramakant},
  booktitle={Thirty-Second AAAI conference on artificial intelligence},
  year={2018}
}



%%%%%%%%%%%%%ù OTHERS %%%%%%%%%%%%%%%%%%%%%

@article{mur2015orb,
  title={ORB-SLAM: a versatile and accurate monocular SLAM system},
  author={Mur-Artal, Raul and Montiel, Jose Maria Martinez and Tardos, Juan D},
  journal={IEEE transactions on robotics},
  volume={31},
  number={5},
  pages={1147--1163},
  year={2015},
  publisher={IEEE}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{sturm2012benchmark,
  title={A benchmark for the evaluation of RGB-D SLAM systems},
  author={Sturm, J{\"u}rgen and Engelhard, Nikolas and Endres, Felix and Burgard, Wolfram and Cremers, Daniel},
  booktitle={2012 IEEE/RSJ international conference on intelligent robots and systems},
  pages={573--580},
  year={2012},
  organization={IEEE}
}

@incollection{pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
}
@inproceedings{heise2013pm,
  title={Pm-huber: Patchmatch with huber regularization for stereo matching},
  author={Heise, Philipp and Klose, Sebastian and Jensen, Brian and Knoll, Alois},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2360--2367},
  year={2013}
}

@INPROCEEDINGS{Geiger2012CVPR,
  author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  title = {Are we ready for Autonomous Driving? The KITTI Vision Benchmark Suite},
  booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
  year = {2012}
}


@article{wang2004image,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P},
  journal={IEEE transactions on image processing},
  volume={13},
  number={4},
  pages={600--612},
  year={2004},
  publisher={IEEE}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}

@article{bommasani2021opportunities,
  title={On the opportunities and risks of foundation models},
  author={Bommasani, Rishi and Hudson, Drew A and Adeli, Ehsan and Altman, Russ and Arora, Simran and von Arx, Sydney and Bernstein, Michael S and Bohg, Jeannette and Bosselut, Antoine and Brunskill, Emma and others},
  journal={arXiv preprint arXiv:2108.07258},
  year={2021}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}


@article{jaderberg2015spatial,
  title={Spatial transformer networks},
  author={Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and others},
  journal={Advances in neural information processing systems},
  volume={28},
  pages={2017--2025},
  year={2015}
}
@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

%%%%%%%%% Transfomers %%%%%%%%%%


@inproceedings{carion2020end,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle={European Conference on Computer Vision},
  pages={213--229},
  year={2020},
  organization={Springer}
}

@article{liu2021we,
  title={Are we ready for a new paradigm shift? A Survey on Visual Deep MLP},
  author={Liu, Ruiyang and Li, Yinghui and Liang, Dun and Tao, Linmi and Hu, Shimin and Zheng, Hai-Tao},
  journal={arXiv preprint arXiv:2111.04060},
  year={2021}
}

@article{hooker2021hardware,
  title={The hardware lottery},
  author={Hooker, Sara},
  journal={Communications of the ACM},
  volume={64},
  number={12},
  pages={58--65},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{radford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  journal={arXiv preprint arXiv:2103.00020},
  year={2021}
}










%%%%%%%%% Transfomers %%%%%%%%%%
@article{cheng2021masked,
  title={Masked-attention mask transformer for universal image segmentation},
  author={Cheng, Bowen and Misra, Ishan and Schwing, Alexander G and Kirillov, Alexander and Girdhar, Rohit},
  journal={arXiv preprint arXiv:2112.01527},
  year={2021}
}
@article{li2021grounded,
  title={Grounded Language-Image Pre-training},
  author={Li, Liunian Harold and Zhang, Pengchuan and Zhang, Haotian and Yang, Jianwei and Li, Chunyuan and Zhong, Yiwu and Wang, Lijuan and Yuan, Lu and Zhang, Lei and Hwang, Jenq-Neng and others},
  journal={arXiv preprint arXiv:2112.03857},
  year={2021}
}

@article{li2021improved,
  title={Improved multiscale vision transformers for classification and detection},
  author={Li, Yanghao and Wu, Chao-Yuan and Fan, Haoqi and Mangalam, Karttikeya and Xiong, Bo and Malik, Jitendra and Feichtenhofer, Christoph},
  journal={arXiv preprint arXiv:2112.01526},
  year={2021}
}

@article{zhai2021scaling,
  title={Scaling vision transformers},
  author={Zhai, Xiaohua and Kolesnikov, Alexander and Houlsby, Neil and Beyer, Lucas},
  journal={arXiv preprint arXiv:2106.04560},
  year={2021}
}

@article{raffel2019exploring,
  title={Exploring the limits of transfer learning with a unified text-to-text transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={arXiv preprint arXiv:1910.10683},
  year={2019}
}
@inproceedings{Vaswani,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 publisher = {Curran Associates, Inc.},
 title = {Attention is All you Need},
 volume = {30},
 year = {2017}
}

@article{Devlin2019,
archivePrefix = {arXiv},
arxivId = {1810.04805},
author = {Devlin, Jacob and Chang, Ming Wei and Lee, Kenton and Toutanova, Kristina},
eprint = {1810.04805},
isbn = {9781950737130},
journal = {NAACL HLT 2019 - 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies - Proceedings of the Conference},
number = {Mlm},
pages = {4171--4186},
title = {{BERT: Pre-training of deep bidirectional transformers for language understanding}},
volume = {1},
year = {2019}
}
@article{Brown2020,
archivePrefix = {arXiv},
arxivId = {2005.14165},
author = {Brown, Tom B. and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel M. and Wu, Jeffrey and Winter, Clemens and Hesse, Christopher and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
eprint = {2005.14165},
issn = {10495258},
journal = {Advances in Neural Information Processing Systems},
title = {{Language models are few-shot learners}},
volume = {2020-December},
year = {2020}
}

@article{dosovitskiy2020,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}
@article{Liu2021,
  title={Swin transformer: Hierarchical vision transformer using shifted windows},
  author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  journal={arXiv preprint arXiv:2103.14030},
  year={2021}
}



%%%% VIDEO FORECASTING %%%%%%%%%%%%%%%%%%%µ

@inproceedings{Eigena,
archivePrefix = {arXiv},
arxivId = {1411.4734},
author = {Eigen, David and Fergus, Rob},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2015.304},
eprint = {1411.4734},
isbn = {9781467383912},
issn = {15505499},
pages = {2650--2658},
title = {{Predicting depth, surface normals and semantic labels with a common multi-scale convolutional architecture}},
volume = {2015 Inter},
year = {2015}
}
@inproceedings{Eigen,
archivePrefix = {arXiv},
arxivId = {1406.2283},
author = {Eigen, David and Puhrsch, Christian and Fergus, Rob},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1406.2283},
issn = {10495258},
pages = {2366--2374},
title = {{Depth map prediction from a single image using a multi-scale deep network}},
volume = {3},
year = {2014}
}


@inproceedings{WilliamLotter2016,
archivePrefix = {arXiv},
arxivId = {1605.07157},
author = {{William Lotter}, Gabriel Kreiman and David Cox},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1605.07157},
issn = {10495258},
pages = {64--72},
title = {{Deep Predictive Coding Networks for Video Prediction and Unsupervised Learning}},
year = {2016}
}
@inproceedings{Wang2020a,
archivePrefix = {arXiv},
arxivId = {2008.05861},
author = {Wang, Jiangliu and Jiao, Jianbo and Liu, Yun Hui},
booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
doi = {10.1007/978-3-030-58520-4_30},
eprint = {2008.05861},
isbn = {9783030585198},
issn = {16113349},
keywords = {Pace,Self-supervised learning,Unsupervised,Video representation},
pages = {504--521},
title = {{ContextVP: Fully Context-Aware Video Prediction}},
volume = {12362 LNCS},
year = {2020}
}
@inproceedings{Finn,
archivePrefix = {arXiv},
arxivId = {1605.07157},
author = {Finn, Chelsea and Goodfellow, Ian and Levine, Sergey},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1605.07157},
issn = {10495258},
pages = {64--72},
title = {{Unsupervised learning for physical interaction through video prediction}},
year = {2016}
}

@article{Kumar2019,
  title={Videoflow: A conditional flow-based model for stochastic video generation},
  author={Kumar, Manoj and Babaeizadeh, Mohammad and Erhan, Dumitru and Finn, Chelsea and Levine, Sergey and Dinh, Laurent and Kingma, Durk},
  journal={arXiv preprint arXiv:1903.01434},
  year={2019}
}

@article{Wu2021a,
archivePrefix = {arXiv},
arxivId = {2103.04174},
author = {Wu, Bohan and Nair, Suraj and Martin-Martin, Roberto and Fei-Fei, Li and Finn, Chelsea},
eprint = {2103.04174},
title = {{Greedy Hierarchical Variational Autoencoders for Large-Scale Video Prediction}},
year = {2021}
}
@inproceedings{Ye2019,
archivePrefix = {arXiv},
arxivId = {1908.08522},
author = {Ye, Yufei and Singh, Maneesh and Gupta, Abhinav and Tulsiani, Shubham},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2019.01045},
eprint = {1908.08522},
isbn = {9781728148038},
issn = {15505499},
pages = {10352--10361},
title = {{Compositional video prediction}},
volume = {2019-Octob},
year = {2019}
}
@inproceedings{Reda2021,
archivePrefix = {arXiv},
arxivId = {1811.00684},
author = {Reda, Fitsum A and Liu, Guilin and Shih, Kevin J and Kirby, Robert and Barker, Jon and Tarjan, David and Tao, Andrew and Catanzaro, Bryan},
booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
doi = {10.1007/978-3-030-01234-2_44},
eprint = {1811.00684},
isbn = {9783030012335},
issn = {16113349},
keywords = {3D CNN,Frame prediction,Optical flow,Sampling kernel},
pages = {747--763},
title = {{SDC-Net: Video prediction using spatially-displaced convolution}},
volume = {11211 LNCS},
year = {2018}
}
@inproceedings{Kalchbrenner2017,
archivePrefix = {arXiv},
arxivId = {1610.00527},
author = {Kalchbrenner, Nal and {Van Den Oord}, A{\"{a}}ron and Simonyan, Karen and Danihelka, Ivo and Vinyals, Oriol and Graves, Alex and Kavukcuoglu, Koray},
booktitle = {34th International Conference on Machine Learning, ICML 2017},
eprint = {1610.00527},
isbn = {9781510855144},
pages = {2821--2829},
title = {{Video pixel networks}},
volume = {4},
year = {2017}
}
@inproceedings{Gao2019,
archivePrefix = {arXiv},
arxivId = {1812.00452},
author = {Gao, Hang and Xu, Huazhe and Cai, Qi Zhi and Wang, Ruth and Yu, Fisher and Darrell, Trevor},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2019.00910},
eprint = {1812.00452},
isbn = {9781728148038},
issn = {15505499},
pages = {9005--9014},
title = {{Disentangling propagation and generation for video prediction}},
volume = {2019-Octob},
year = {2019}
}
@inproceedings{Babaeizadeh2018,
archivePrefix = {arXiv},
arxivId = {1710.11252},
author = {Babaeizadeh, Mohammad and Finn, Chelsea and Erhan, Dumitru and Campbell, Roy and Levine, Sergey},
booktitle = {6th International Conference on Learning Representations, ICLR 2018 - Conference Track Proceedings},
eprint = {1710.11252},
isbn = {1710.11252v2},
title = {{Stochastic variational video prediction}},
year = {2018}
}
@inproceedings{Denton2018,
archivePrefix = {arXiv},
arxivId = {1802.07687},
author = {Denton, Emily and Fergus, Rob},
booktitle = {35th International Conference on Machine Learning, ICML 2018},
eprint = {1802.07687},
isbn = {9781510867963},
pages = {1906--1919},
title = {{Stochastic Video Generation with a Learned Prior}},
volume = {3},
year = {2018}
}
@article{Yan2021,
archivePrefix = {arXiv},
arxivId = {2104.10157},
author = {Yan, Wilson and Zhang, Yunzhi and Abbeel, Pieter and Srinivas, Aravind},
eprint = {2104.10157},
title = {{VideoGPT: Video Generation using VQ-VAE and Transformers}},
year = {2021}
}


@article{Walker2021,
  title={Predicting Video with VQVAE},
  author={Walker, Jacob and Razavi, Ali and Oord, A{\"a}ron van den},
  journal={arXiv preprint arXiv:2103.01950},
  year={2021}
}


@inproceedings{Wu2021,
  title={MotionRNN: A flexible model for video prediction with spacetime-varying motions},
  author={Wu, Haixu and Yao, Zhiyu and Wang, Jianmin and Long, Mingsheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15435--15444},
  year={2021}
}






%%%% SEMANTIC FORECASTING %%%%%%%%%%%%%%%%%%%µ


@inproceedings{Terwilliger2019,
archivePrefix = {arXiv},
arxivId = {1809.08318},
author = {Terwilliger, Adam M and Brazil, Garrick and Liu, Xiaoming},
booktitle = {Proceedings - 2019 IEEE Winter Conference on Applications of Computer Vision, WACV 2019},
doi = {10.1109/WACV.2019.00186},
eprint = {1809.08318},
isbn = {9781728119755},
pages = {1703--1712},
title = {{Recurrent flow-guided semantic forecasting}},
year = {2019}
}


@inproceedings{Bhattacharyya2019,
archivePrefix = {arXiv},
arxivId = {1810.00746},
author = {Bhattacharyya, Apratim and Fritz, Mario and Schiele, Bernt},
booktitle = {7th International Conference on Learning Representations, ICLR 2019},
eprint = {1810.00746},
title = {{Bayesian prediction of future street scenes using synthetic likelihoods}},
year = {2019}
}


@inproceedings{Luc2017,
archivePrefix = {arXiv},
arxivId = {1703.07684},
author = {Luc, Pauline and Neverova, Natalia and Couprie, Camille and Verbeek, Jakob and Lecun, Yann},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
doi = {10.1109/ICCV.2017.77},
eprint = {1703.07684},
isbn = {9781538610329},
issn = {15505499},
pages = {648--657},
title = {{Predicting Deeper into the Future of Semantic Segmentation}},
volume = {2017-Octob},
year = {2017}
}


@inproceedings{Graber2021,
archivePrefix = {arXiv},
arxivId = {2104.03962},
author = {Graber, Colin and Tsai, Grace and Firman, Michael and Brostow, Gabriel and Schwing, Alexander},
booktitle = {IEEE Computer Society Conference on Computer Vision and Pattern Recognition Workshops},
doi = {10.1109/CVPRW53098.2021.00257},
eprint = {2104.03962},
isbn = {9781665448994},
issn = {21607516},
pages = {2279--2288},
title = {{Panoptic segmentation forecasting}},
year = {2021}
}


@article{Chiu2020,
archivePrefix = {arXiv},
arxivId = {1904.10666},
author = {Chiu, Hsu Kuang and Adeli, Ehsan and Niebles, Juan Carlos},
doi = {10.1109/LRA.2020.2992184},
eprint = {1904.10666},
issn = {23773766},
journal = {IEEE Robotics and Automation Letters},
keywords = {Computer vision for transportation,deep learning for visual perception,semantic scene understanding,visual learning},
number = {3},
pages = {4202--4209},
title = {{Segmenting the Future}},
volume = {5},
year = {2020}
}



@inproceedings{Saric2020,
author = {Saric, Josip and Orsic, Marin and Antunovic, Tonci and Vrazic, Sacha and Segvic, Sinisa},
booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
doi = {10.1109/CVPR42600.2020.01066},
issn = {10636919},
pages = {10645--10654},
title = {{Warp to the Future: Joint Forecasting of Features and Feature Motion}},
year = {2020}
}
@article{Mathieu2016,
  title={Deep multi-scale video prediction beyond mean square error},
  author={Mathieu, Michael and Couprie, Camille and LeCun, Yann},
  journal={arXiv preprint arXiv:1511.05440},
  year={2015}
}

@inproceedings{Rakhimov,
archivePrefix = {arXiv},
arxivId = {2006.10704},
author = {Rakhimov, Ruslan and Volkhonskiy, Denis and Artemov, Alexey and Zorin, Denis and Burnaev, Evgeny},
booktitle = {VISIGRAPP 2021 - Proceedings of the 16th International Joint Conference on Computer Vision, Imaging and Computer Graphics Theory and Applications},
doi = {10.5220/0010241801010112},
eprint = {2006.10704},
isbn = {9789897584886},
keywords = {Deep learning,Generative adversarial networks,Video generation},
pages = {101--112},
title = {{Latent video transformer}},
volume = {5},
year = {2021}
}


%%%% DEPTH FORECASTING %%%%%%%%%%%%%%%%%%%µ



@article{weng2020inverting,
  title={Inverting the Pose Forecasting Pipeline with SPF2: Sequential Pointcloud Forecasting for Sequential Pose Forecasting},
  author={Weng, Xinshuo and Wang, Jianren and Levine, Sergey and Kitani, Kris and Rhinehart, Nicholas},
  journal={arXiv preprint arXiv:2003.08376},
  year={2020}
}

@inproceedings{Mahjourian2017,
archivePrefix = {arXiv},
arxivId = {1609.06377},
author = {Mahjourian, Reza and Wicke, Martin and Angelova, Anelia},
booktitle = {IEEE Intelligent Vehicles Symposium, Proceedings},
doi = {10.1109/IVS.2017.7995953},
eprint = {1609.06377},
isbn = {9781509048045},
pages = {1700--1707},
title = {{Geometry-based next frame prediction from monocular video}},
year = {2017}
}

@inproceedings{Qi2019,
author = {Qi, Xiaojuan and Liu, Zhengzhe and Chen, Qifeng and Jia, Jiaya},
booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
doi = {10.1109/CVPR.2019.00786},
isbn = {9781728132938},
issn = {10636919},
keywords = {Image and Video Synthesis,RGBD sensors and analytics},
pages = {7665--7674},
title = {{3D motion decomposition for RGBD future dynamic scene synthesis}},
volume = {2019-June},
year = {2019}
}

@inproceedings{Hu2020,
archivePrefix = {arXiv},
arxivId = {2003.06409},
author = {Hu, Anthony and Cotter, Fergal and Mohan, Nikhil and Gurau, Corina and Kendall, Alex},
booktitle = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
doi = {10.1007/978-3-030-58517-4_45},
eprint = {2003.06409},
isbn = {9783030585167},
issn = {16113349},
pages = {767--785},
title = {{Probabilistic Future Prediction for Video Scene Understanding}},
volume = {12361 LNCS},
year = {2020}
}
@article{boulahbal2022instance,
  title={Instance-aware multi-object self-supervision for monocular depth prediction},
  author={Boulahbal, Houssem Eddine and Voicila, Adrian and Comport, Andrew I},
  journal={IEEE Robotics and Automation Letters},
  volume={7},
  number={4},
  pages={10962--10968},
  year={2022},
  publisher={IEEE}
}
@inproceedings{boulahbal2022forecasting,
  title={Forecasting of depth and ego-motion with transformers and self-supervision},
  author={Boulahbal, Houssem Eddine and Voicila, Adrian and Comport, Andrew I},
  booktitle={2022 26th International Conference on Pattern Recognition (ICPR)},
  pages={3706--3713},
  year={2022},
  organization={IEEE}
}


@inproceedings{guizilini2022multi,
  title={Multi-frame self-supervised depth with transformers},
  author={Guizilini, Vitor and Ambruș, Rareș and Chen, Dian and Zakharov, Sergey and Gaidon, Adrien},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={160--170},
  year={2022}
}
@ARTICLE{9864127,
  author={Hwang, Seung-Jun and Park, Sung-Jun and Baek, Joong-Hwan and Kim, Byungkyu},
  journal={IEEE Sensors Journal}, 
  title={Self-Supervised Monocular Depth Estimation Using Hybrid Transformer Encoder}, 
  year={2022},
  volume={22},
  number={19},
  pages={18762-18770},
  doi={10.1109/JSEN.2022.3199265}}

%%%% DEPTH ESTIMATION %%%%%%%%%%%%%%%%%%%µ
@article{Yin2018,
archivePrefix = {arXiv},
arxivId = {1803.02276},
author = {Yin, Zhichao and Shi, Jianping},
doi = {10.1109/CVPR.2018.00212},
eprint = {1803.02276},
isbn = {9781538664209},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {1983--1992},
title = {{GeoNet: Unsupervised Learning of Dense Depth, Optical Flow and Camera Pose}},
year = {2018}
}
@article{Shu2020,
archivePrefix = {arXiv},
arxivId = {2007.10603},
author = {Shu, Chang and Yu, Kun and Duan, Zhixiang and Yang, Kuiyuan},
doi = {10.1007/978-3-030-58529-7_34},
eprint = {2007.10603},
isbn = {9783030585280},
issn = {16113349},
journal = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
pages = {572--588},
title = {{Feature-Metric Loss for Self-supervised Learning of Depth and Egomotion}},
volume = {12364 LNCS},
year = {2020}
}

@article{Wang2021,
author = {Wang, Lijun and Wang, Yifan and Wang, Linzhao and Zhan, Yunlong and Wang, Ying and Lu, Huchuan},
journal = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
pages = {12727--12736},
title = {{Can Scale-Consistent Monocular Depth Be Learned in a Self-Supervised Scale-Invariant Manner?}},
year = {2021}
}

@inproceedings{Ranjan2019,
arxivId = {1805.09806},
author = {Ranjan, Anurag and Jampani, Varun and Balles, Lukas and Kim, Kihwan and Sun, Deqing and Wulff, Jonas and Black, Michael J},
booktitle = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
doi = {10.1109/CVPR.2019.01252},
eprint = {1805.09806},
isbn = {9781728132938},
issn = {10636919},
keywords = {Deep Learning,Low-level Vision},
pages = {12232--12241},
title = {{Competitive collaboration: Joint unsupervised learning of depth, camera motion, optical flow and motion segmentation}},
volume = {2019-June},
year = {2019}
}



@article{Yang2021,
archivePrefix = {arXiv},
arxivId = {2103.12091},
author = {Yang, Guanglei and Tang, Hao and Ding, Mingli and Sebe, Nicu and Ricci, Elisa},
eprint = {2103.12091},
pages = {16269--16279},
title = {{Transformer-Based Attention Networks for Continuous Pixel-Wise Prediction}},
year = {2021}
}
@article{Gordon2019,
archivePrefix = {arXiv},
arxivId = {1904.04998},
author = {Gordon, Ariel and Li, Hanhan and Jonschkowski, Rico and Angelova, Anelia},
doi = {10.1109/ICCV.2019.00907},
eprint = {1904.04998},
isbn = {9781728148038},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
pages = {8976--8985},
title = {{Depth from videos in the wild: Unsupervised monocular depth learning from unknown cameras}},
volume = {2019-Octob},
year = {2019}
}
@article{Kendall2015,
archivePrefix = {arXiv},
arxivId = {1505.07427},
author = {Kendall, Alex and Grimes, Matthew and Cipolla, Roberto},
doi = {10.1109/ICCV.2015.336},
eprint = {1505.07427},
isbn = {9781467383912},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
pages = {2938--2946},
title = {{PoseNet: A convolutional network for real-time 6-dof camera relocalization}},
volume = {2015 Inter},
year = {2015}
}
@article{Jaderberg2015,
archivePrefix = {arXiv},
arxivId = {1506.02025},
author = {Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and Kavukcuoglu, Koray},
eprint = {1506.02025},
issn = {10495258},
journal = {Advances in Neural Information Processing Systems},
pages = {2017--2025},
title = {{Spatial transformer networks}},
volume = {2015-Janua},
year = {2015}
}
@article{Mahjourian2018,
archivePrefix = {arXiv},
arxivId = {1802.05522},
author = {Mahjourian, Reza and Wicke, Martin and Angelova, Anelia},
doi = {10.1109/CVPR.2018.00594},
eprint = {1802.05522},
isbn = {9781538664209},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {5667--5675},
title = {{Unsupervised Learning of Depth and Ego-Motion from Monocular Video Using 3D Geometric Constraints}},
year = {2018}
}
@article{Liu2016,
archivePrefix = {arXiv},
arxivId = {1502.07411},
author = {Liu, Fayao and Shen, Chunhua and Lin, Guosheng and Reid, Ian},
doi = {10.1109/TPAMI.2015.2505283},
eprint = {1502.07411},
issn = {01628828},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
keywords = {Depth estimation,conditional random field (CRF),deep convolutional neural networks (CNN),fully convolutional networks,superpixel pooling},
number = {10},
pages = {2024--2039},
title = {{Learning Depth from Single Monocular Images Using Deep Convolutional Neural Fields}},
volume = {38},
year = {2016}
}


@article{Chen2016,
  title={Single-image depth perception in the wild},
  author={Chen, Weifeng and Fu, Zhao and Yang, Dawei and Deng, Jia},
  journal={Advances in neural information processing systems},
  volume={29},
  pages={730--738},
  year={2016}
}

@article{Godard2017,
archivePrefix = {arXiv},
arxivId = {1609.03677},
author = {Godard, Cl{\'{e}}ment and {Mac Aodha}, Oisin and Brostow, Gabriel J.},
doi = {10.1109/CVPR.2017.699},
eprint = {1609.03677},
isbn = {9781538604571},
issn = {1063-6919},
journal = {Proceedings - 30th IEEE Conference on Computer Vision and Pattern Recognition, CVPR 2017},
pages = {6602--6611},
title = {{Unsupervised monocular depth estimation with left-right consistency}},
volume = {2017-January},
year = {2017}
}
@article{Zhou2017,
archivePrefix = {arXiv},
arxivId = {1704.07813},
author = {Zhou, Tinghui and Brown, Matthew and Snavely, Noah and Lowe, David G.},
doi = {10.1109/CVPR.2017.700},
eprint = {1704.07813},
isbn = {9781538604571},
journal = {Proceedings - 30th IEEE Conference on Computer Vision and Pattern Recognition, CVPR 2017},
pages = {6612--6621},
title = {{Unsupervised learning of depth and ego-motion from video}},
volume = {2017-January},
year = {2017}
}
@inproceedings{garg2016unsupervised,
  title={Unsupervised cnn for single view depth estimation: Geometry to the rescue},
  author={Garg, Ravi and Bg, Vijay Kumar and Carneiro, Gustavo and Reid, Ian},
  booktitle={European conference on computer vision},
  pages={740--756},
  year={2016},
  organization={Springer}
}
@article{Zhan2018,
archivePrefix = {arXiv},
arxivId = {1803.03893},
author = {Zhan, Huangying and Garg, Ravi and Weerasekera, Chamara Saroj and Li, Kejie and Agarwal, Harsh and Reid, Ian M.},
doi = {10.1109/CVPR.2018.00043},
eprint = {1803.03893},
isbn = {9781538664209},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {340--349},
title = {{Unsupervised Learning of Monocular Depth Estimation and Visual Odometry with Deep Feature Reconstruction}},
year = {2018}
}
@article{Godard2019,
archivePrefix = {arXiv},
arxivId = {1806.01260},
author = {Godard, Clement and Aodha, Oisin Mac and Firman, Michael and Brostow, Gabriel},
doi = {10.1109/ICCV.2019.00393},
eprint = {1806.01260},
isbn = {9781728148038},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
number = {1},
pages = {3827--3837},
title = {{Digging into self-supervised monocular depth estimation}},
volume = {2019-October},
year = {2019}
}
@article{Chen2019,
archivePrefix = {arXiv},
arxivId = {1907.05820},
author = {Chen, Yuhua and Schmid, Cordelia and Sminchisescu, Cristian},
doi = {10.1109/ICCV.2019.00716},
eprint = {1907.05820},
isbn = {9781728148038},
issn = {15505499},
journal = {Proceedings of the IEEE International Conference on Computer Vision},
pages = {7062--7071},
title = {{Self-supervised learning with geometric constraints in monocular video: Connecting flow, depth, and camera}},
volume = {2019-October},
year = {2019}
}
@article{Lee2019,
archivePrefix = {arXiv},
arxivId = {1909.06999},
author = {Lee, Seokju and Im, Sunghoon and Lin, Stephen and Kweon, In So},
doi = {10.1109/IROS40897.2019.8967970},
eprint = {1909.06999},
isbn = {9781728140049},
issn = {21530866},
journal = {IEEE International Conference on Intelligent Robots and Systems},
pages = {1180--1186},
title = {{Learning Residual Flow as Dynamic Motion from Stereo Videos}},
year = {2019}
}
@article{Johnston2020,
archivePrefix = {arXiv},
arxivId = {2003.13951},
author = {Johnston, Adrian and Carneiro, Gustavo},
doi = {10.1109/CVPR42600.2020.00481},
eprint = {2003.13951},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {4755--4764},
title = {{Self-supervised monocular trained depth estimation using self-attention and discrete disparity volume}},
year = {2020}
}
@article{Klingner2020,
archivePrefix = {arXiv},
arxivId = {2007.06936},
author = {Klingner, Marvin and Term{\"{o}}hlen, Jan Aike and Mikolajczyk, Jonas and Fingscheidt, Tim},
doi = {10.1007/978-3-030-58565-5_35},
eprint = {2007.06936},
isbn = {9783030585648},
issn = {16113349},
journal = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
pages = {582--600},
title = {{Self-supervised Monocular Depth Estimation: Solving the Dynamic Object Problem by Semantic Guidance}},
volume = {12365 LNCS},
year = {2020}
}
@inproceedings{wimbauer2021monorec,
  title={MonoRec: Semi-supervised dense reconstruction in dynamic environments from a single moving camera},
  author={Wimbauer, Felix and Yang, Nan and Von Stumberg, Lukas and Zeller, Niclas and Cremers, Daniel},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={6112--6122},
  year={2021}
}
@article{Bian2019,
  title={Unsupervised scale-consistent depth and ego-motion learning from monocular video},
  author={Bian, Jiawang and Li, Zhichao and Wang, Naiyan and Zhan, Huangying and Shen, Chunhua and Cheng, Ming-Ming and Reid, Ian},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={35--45},
  year={2019}
}
@inproceedings{Watson2021,
  title={The Temporal Opportunist: Self-Supervised Multi-Frame Monocular Depth},
  author={Watson, Jamie and Mac Aodha, Oisin and Prisacariu, Victor and Brostow, Gabriel and Firman, Michael},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1164--1174},
  year={2021}
}

@article{Boulahbal2021,
  title={Are conditional GANs explicitly conditional?},
  author={Boulahbal, Houssem-eddine and Voicila, Adrian and Comport, Andrew},
  journal={arXiv preprint arXiv:2106.15011},
  year={2021}
}
@inproceedings{Almalioglu2019,
archivePrefix = {arXiv},
arxivId = {1809.05786},
author = {Almalioglu, Yasin and Saputra, Muhamad Risqi U. and {De Gusmao}, Pedro P.B. and Markham, Andrew and Trigoni, Niki},
booktitle = {Proceedings - IEEE International Conference on Robotics and Automation},
doi = {10.1109/ICRA.2019.8793512},
eprint = {1809.05786},
isbn = {9781538660263},
issn = {10504729},
pages = {5474--5480},
title = {{GANVO: Unsupervised deep monocular visual odometry and depth estimation with generative adversarial networks}},
volume = {2019-May},
year = {2019}
}
@article{Lee2019a,
archivePrefix = {arXiv},
arxivId = {1907.10326},
author = {Lee, Jin Han and Han, Myung-kyu and Ko, Dong Wook and Suh, Il Hong},
eprint = {1907.10326},
issn = {2331-8422},
title = {{From Big to Small: Multi-Scale Local Planar Guidance for Monocular Depth Estimation}},
url = {http://arxiv.org/abs/1907.10326},
year = {2019}
}
@article{Rares2020,
archivePrefix = {arXiv},
arxivId = {1905.02693},
author = {Rares, Vitor Guizilini and Ambrus and Pillai, Sudeep and Raventos, Allan and Gaidon, Adrien},
doi = {10.1109/CVPR42600.2020.00256},
eprint = {1905.02693},
issn = {10636919},
journal = {Proceedings of the IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
pages = {2482--2491},
title = {{3D packing for self-supervised monocular depth estimation}},
year = {2020}
}
@article{Li2021,
archivePrefix = {arXiv},
arxivId = {2101.02143},
author = {Li, Xiangyu and Hou, Yonghong and Wang, Pichao and Gao, Zhimin and Xu, Mingliang and Li, Wanqing},
doi = {10.1007/s00521-020-05545-8},
eprint = {2101.02143},
issn = {14333058},
journal = {Neural Computing and Applications},
keywords = {Geometry constraint,Transformer,Unsupervised learning,Visual odometry},
number = {13},
pages = {8031--8042},
title = {{Transformer guided geometry model for flow-based unsupervised visual odometry}},
volume = {33},
year = {2021}
}



%%%%%%%%%%%%%ù OTHERS %%%%%%%%%%%%%%%%%%%%%

@article{mur2015orb,
  title={ORB-SLAM: a versatile and accurate monocular SLAM system},
  author={Mur-Artal, Raul and Montiel, Jose Maria Martinez and Tardos, Juan D},
  journal={IEEE transactions on robotics},
  volume={31},
  number={5},
  pages={1147--1163},
  year={2015},
  publisher={IEEE}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{sturm2012benchmark,
  title={A benchmark for the evaluation of RGB-D SLAM systems},
  author={Sturm, J{\"u}rgen and Engelhard, Nikolas and Endres, Felix and Burgard, Wolfram and Cremers, Daniel},
  booktitle={2012 IEEE/RSJ international conference on intelligent robots and systems},
  pages={573--580},
  year={2012},
  organization={IEEE}
}

@incollection{pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
}
@inproceedings{heise2013pm,
  title={Pm-huber: Patchmatch with huber regularization for stereo matching},
  author={Heise, Philipp and Klose, Sebastian and Jensen, Brian and Knoll, Alois},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2360--2367},
  year={2013}
}

@article{RobotCarDatasetIJRR,
  Author = {Will Maddern and Geoff Pascoe and Chris Linegar and Paul Newman},
  Title = {{1 Year, 1000km: The Oxford RobotCar Dataset}},
  Journal = {The International Journal of Robotics Research (IJRR)},
  Volume = {36},
  Number = {1},
  Pages = {3-15},
  Year = {2017},
  doi = {10.1177/0278364916679498},
  }

  
@INPROCEEDINGS{Geiger2012CVPR,
  author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  title = {Are we ready for Autonomous Driving? The KITTI Vision Benchmark Suite},
  booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
  year = {2012}
}

@inproceedings{liu2021swin,
  title={Swin transformer: Hierarchical vision transformer using shifted windows},
  author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={10012--10022},
  year={2021}
}

@article{wang2004image,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Wang, Zhou and Bovik, Alan C and Sheikh, Hamid R and Simoncelli, Eero P},
  journal={IEEE transactions on image processing},
  volume={13},
  number={4},
  pages={600--612},
  year={2004},
  publisher={IEEE}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}

@article{bommasani2021opportunities,
  title={On the opportunities and risks of foundation models},
  author={Bommasani, Rishi and Hudson, Drew A and Adeli, Ehsan and Altman, Russ and Arora, Simran and von Arx, Sydney and Bernstein, Michael S and Bohg, Jeannette and Bosselut, Antoine and Brunskill, Emma and others},
  journal={arXiv preprint arXiv:2108.07258},
  year={2021}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}
@inproceedings{jaderberg2015spatial,
  title={Spatial transformer networks},
  author={Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and Kavukcuoglu, Koray},
  booktitle={Proceedings of the 28th International Conference on Neural Information Processing Systems-Volume 2},
  pages={2017--2025},
  year={2015}
}


@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

%%%%%%%%% Transfomers %%%%%%%%%%


@inproceedings{carion2020end,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle={European Conference on Computer Vision},
  pages={213--229},
  year={2020},
  organization={Springer}
}

@article{liu2021we,
  title={Are we ready for a new paradigm shift? A Survey on Visual Deep MLP},
  author={Liu, Ruiyang and Li, Yinghui and Liang, Dun and Tao, Linmi and Hu, Shimin and Zheng, Hai-Tao},
  journal={arXiv preprint arXiv:2111.04060},
  year={2021}
}

@article{hooker2021hardware,
  title={The hardware lottery},
  author={Hooker, Sara},
  journal={Communications of the ACM},
  volume={64},
  number={12},
  pages={58--65},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{radford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  journal={arXiv preprint arXiv:2103.00020},
  year={2021}
}

==> video-depth/results_ablation.tex <==
 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c |}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$&
\hline \hline


E1 &  & & & &                       
0.114  &   0.809  &   4.702  &   0.187  &   0.875  &   0.961  &   0.983     \\ 

E2 & \checkmark & & & &             
0.113  &   0.860  &   4.812  &   0.190  &   0.870  &   0.958  &   0.982    \\

E3 &  & \checkmark & & &           
0.110  &   0.805  &   4.678  &   0.187  &   0.879  &   0.961  &   0.983   \\



E4 & \checkmark  & \checkmark & & &     
0.112  &   0.844  &   4.754  &   0.189  &   0.876  &   0.960  &   0.981  \\

\hline \hline 

E5 &  & & \checkmark& &            
0.118  &   0.905  &   4.881  &   0.194  &   0.868  &   0.957  &   0.981  \\

E6 &  & & &\checkmark &             
0.110  &   0.765  &   4.809  &   0.192  &   0.876  &   0.957  &   0.981    \\

E7 & \checkmark &  & &\checkmark &             
0.110  &   0.770  &   4.884  &   0.193  &   0.877  &   0.957  &   0.980 \\

E8 & & \checkmark  & &  \checkmark  &             
 0.109  &   0.762  &   4.811  &   0.191  &   0.877  &   0.957  &   0.981   \\

\hline 

\end{tabular}
\caption{$t=0$ Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}




 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c|}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline  
E1 &  & & & &                       
0.125  &   0.994  &   4.986  &   0.201  &   0.859  &   0.954  &   0.980   \\ 

E2 & \checkmark & & & &             
 0.124  &   1.038  &   5.128  &   0.205  &   0.855  &   0.950  &   0.978    \\

E3 &  & \checkmark & & &           
0.121  &   0.989  &   5.026  &   0.203  &   0.863  &   0.951  &   0.978   \\



E4 & \checkmark  & \checkmark & &  &            
  0.125  &   1.082  &   5.191  &   0.207  &   0.859  &   0.950  &   0.977     \\

\hline \hline 
E5 &  & & \checkmark& &            
0.129  &   1.124  &   5.244  &   0.209  &   0.851  &   0.948  &   0.976    \\

E6 &  & & &\checkmark &             
0.118  &   0.871  &   5.034  &   0.204  &   0.864  &   0.951  &   0.978     \\

E7 & \checkmark  & & &\checkmark &             
0.118  &   0.887  &   5.112  &   0.204  &   0.864  &   0.950  &   0.977  \\
E8 &  & \checkmark & &  \checkmark  &             
 0.116  &   0.848  &   4.951  &   0.200  &   0.868  &   0.953  &   0.978  \\

\hline \hline

\end{tabular}
\caption{$t=1$  Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}



 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c|}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline
E1 &  & & & &                       
 0.148  &   1.300  &   5.468  &   0.226  &   0.823  &   0.939  &   0.972     \\ 

E2 & \checkmark & & & &             
 0.146  &   1.317  &   5.553  &   0.227  &   0.823  &   0.935  &   0.971    \\

E3 &  & \checkmark & & &           
   0.146  &   1.295  &   5.493  &   0.227  &   0.824  &   0.935  &   0.971   \\



E4 & \checkmark  & \checkmark & &  &            
0.147  &   1.363  &   5.624  &   0.230  &   0.824  &   0.935  &   0.970   \\

\hline \hline 
E5 &  & & \checkmark& &            
 0.152  &   1.485  &   5.744  &   0.233  &   0.818  &   0.933  &   0.970    \\

E6 &  & & &\checkmark &             
0.137  &   1.106  &   5.407  &   0.223  &   0.833  &   0.938  &   0.972 \\

E7 &\checkmark  &  & &\checkmark &             
0.136  &   1.128  &   5.456  &   0.224  &   0.833  &   0.937  &   0.971 \\

E8 &  &\checkmark & &  \checkmark  &             
 0.137  &   1.106  &   5.342  &   0.221  &   0.834  &   0.939  &   0.972  \\

\hline 

\end{tabular}
\caption{$t=3$  Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}






 \begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c ||c c c c| c c c|}
\hline 
experiment & Use vae & share prediction & Instance warping & stereo &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline

ForecastMonodepth2 & & & & &
0.201  &   1.588   &   0.275  &   6.166 &   0.702 &  0.897  &   0.960\\
ICPR paper & & & & &
0.178  &  1.645   &   0.257 &   6.196 &   0.761  &   0.914  &   0.964 \\
\hline \hline

E1 &  & & & &                       
0.167  &   1.545  &   5.851  &   0.243  &   0.793  &   0.926  &   0.967 \\ 

E2 & \checkmark & & & &             
0.166  &   1.563  &   5.909  &   0.244  &   0.790  &   0.923  &   0.966    \\

E3 &  & \checkmark & & &           
0.165  &   1.489  &   5.805  &   0.245  &   0.792  &   0.921  &   0.964   \\



E4 & \checkmark  & \checkmark & &  &            
0.168  &   1.624  &   5.968  &   0.248  &   0.791  &   0.922  &   0.965    \\

\hline \hline 

E5 &  & & \checkmark& &            
0.170  &   1.711  &   6.082  &   0.250  &   0.788  &   0.920  &   0.964    \\

E6 &  & & &\checkmark &             
 0.156  &   1.312  &   5.720  &   0.242  &   0.799  &   0.924  &   0.966    \\

E7 & \checkmark &  & &\checkmark &             
0.155  &   1.328  &   5.792  &   0.241  &   0.799  &   0.925  &   0.967 \\

E8 &  & \checkmark & &  \checkmark  &             
 0.153  &   1.323  &   5.730  &   0.239  &   0.803  &   0.926  &   0.967    \\

\hline 

\end{tabular}
\caption{$t=5$  Quantitative performance comparison of on the KITTI benchmark.}
%\caption{Quantitative performance comparison of on the KITTI benchmark with Eigen split~\cite{Geiger2012CVPR}. For Abs Rel, Sq Rel, RMSE and RMSE log lower is better, and for $\delta < 1.25$, $\delta < 1.25^2$ and $\delta < 1.25^3$ higher is better. The Supervision column illustrates the traing modalities: (M) raw images (S)Semantic, (F) optical flow, (TS) Teacher-student. At test-time, all monocular methods (M) scale the estimated depths with median ground-truth LiDAR.The best scores are bold and the second are underlined}
\label{tab:results}
\end{table*}

==> video-depth/results_generalization.tex <==


\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l |cc||c c c c ||c c c|}
\hline
Method & Known intrinsic & Resolution &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline  
Manydepth~\cite{}& \checkmark
 & 640$\times$192  & 0.098 & 0.770 & 4.459 & 0.176 & 0.900& 0.965 & 0.983 \\\text
 Manydepth~\cite{}& 
 & 640$\times$192  &  0.112  &   0.839  &   4.626  &   0.187  &   0.881  &   0.962  &   0.983  \\
  \hline \hline
DepthFormer~\cite{}& \checkmark   & 640$\times$192  & 0.090 & 0.661 & 4.149 & 0.175  & 0.905 & 0.967  & 0.984 \\
DepthFormer~\cite{}&  & 640$\times$192  & 0.125   &  0.893   &  4.713   &  0.206 & 0.849   & 0.949 &  0.977 \\
 \hline \hline
Ours& & 640$\times$192 & 0.107  &   0.797  &   4.614  &   0.185  &   0.889  &   0.963  &   0.982  \\
\hline 

\end{tabular}
\caption{Quantitative performance comparison of on the KITTI benchmark.}
\label{tab:results}
\end{table*}




\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l| c||c c c c |c c c|}
\hline  
Method& Known intrinsic  &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline  \hline  
Manydepth~\cite{}& \checkmark  & 0.169  &   1.787  &   8.352  &   0.236  &   0.749  &   0.932  &   0.978  \\
Manydepth~\cite{}&  & 0.165  &   1.749  &   8.304  &   0.232  &   0.761  &   0.933  &   0.978 \\

DepthFormer~\cite{} &\checkmark &   0.213  &   2.291  &   8.978  &   0.292  &   0.633  &   0.877  &   0.957  \\

DepthFormer~\cite{}&   &  0.177  &   2.022  &   8.840  &   0.257  &   0.727  &   0.902  &   0.963  \\
Ours&  & 0.153  &   1.792  &   8.890  &   0.235  &   0.771  &   0.920  &   0.974  \\
\hline 

\end{tabular}
\caption{Quantitative performance comparison of on the Cityscapes.}
\label{tab:results}
\end{table*}




\begin{table*}
\centering
\footnotesize
\begin{tabular}{|l||c c c c c c c c|}
\hline 
Conditions & Method  &Abs Rel& Sq Rel&  RMSE & RMSE log  &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\\
\hline \hline
\multirow{3}{*}{\textbf{Rain sequence}} 
& Manydepth~\cite{} & 0.325  &   3.622  &   8.300  &   0.342  &   0.519  &   0.781  &   0.919  \\
& DepthFormer~\cite{} & 0.438  &   5.596  &   9.618  &   0.437  &   0.468  &   0.698  &   0.838  \\
& Ours& 0.284  &   3.064  &   7.934  &   0.313  &   0.561  &   0.821  &   0.937  \\
\hline

%\multirow{3}{*}{\textbf{Night sequence}} 
%& Manydepth~\cite{} &   0.422  &   5.304  &  11.154  &   0.451  &   0.408  &   0.664  &   0.834  \\
%& DepthFormer~\cite{}& 0.562  &   7.935  &  11.245  &   0.548  &   0.388  &   0.636  &   0.783  \\
%& Ours&      0.348  &   4.294  &  10.832  &   0.395  &   0.455  &   0.708  &   0.881  \\
%\hline \hline
\multirow{3}{*}{\textbf{Snow sequence}} 
& Manydepth~\cite{} &   0.328  &   3.694  &   8.712  &   0.367  &   0.505  &   0.766  &   0.902  \\
& DepthFormer~\cite{}&   0.441  &   5.551  &   9.486  &   0.448  &   0.477  &   0.718  &   0.844  \\
& Ours&     0.276  &   2.818  &   8.183  &   0.328  &   0.544  &   0.813  &   0.935  \\
\hline \hline


\multirow{3}{*}{\textbf{Overcast sequence}} 
& Manydepth~\cite{} &   0.247  &   3.018  &   6.442  &   0.278  &   0.668  &   0.836  &   0.924  \\
& DepthFormer~\cite{}& 0.359  &   4.980  &   7.167  &   0.357  &   0.606  &   0.769  &   0.865  \\
& Ours&      0.238  &   2.979  &   6.725  &   0.278  &   0.670  &   0.832  &   0.926  \\
\hline 

\end{tabular}
\caption{Quantitative performance comparison of on the Robotcar dataset night sequence}
\label{tab:results}
\end{table*}

